Properties of coplanar periodic electrodes in confined spaces: Case of two-dimensional diffusion

Periodic configurations of electrodes, in particular of microelectrodes, have been of interest since the advent of microfabrication. In this report, theory which is common to any periodic cell (or any cell that can be extended periodically) with finite height and two-dimensional symmentry was derived. The diffusion equation in this cell was solved and the concentration profile was obtained in terms of its Fourier coefficients and as a function of an arbitrary current density. From this base result, a set of properties were derived which are fairly general, since they don't assume restrictions such as reversible electrode reactions (Nernst equation valid when current circulates). These properties involve: horizontal averages and (weighted) sum of concentrations, both with a close connection to the net current and accumulation of species in the cell. The derived properties allow: to explain qualitative aspects of collection efficiency and limiting currents, to predict the concentration on counter electrodes and non-linearities caused by depletion of species at extremely polarized electrodes, and to estimate the time required by the current to reach steady state in potential controlled experiments. The theoretical results are illustrated analytically and numerically for the concrete case of interdigitated array of electrodes.

==> text-additional_proofs.tex <==
% !TeX root = article
% !TeX encoding = utf8
% !TeX spellcheck = en_US


\section{Additional proofs}

\subsection{Lemma \ref{coplanar:lem:g-h}}

In the proof below it is found how to obtain the principal parts
$\tilde{G}(z,s)$ and $\tilde{G}(z,s)^{-1}$ of $G(z,s)$ and $G(z,s)^{-1}$ through residues.

Since the number of poles of $G(z,s)$ and $G(z,s)^{-1}$ is infinite,
the the principal parts $\tilde{G}(z,s)$ and $\tilde{G}(z,s)^{-1}$
may not agree with the original functions $G(z,s)$ and $G(z,s)^{-1}$.

The agreement between $F(z,s) - \tilde{F}(z,s)$ with $F \in \{G, G^{-1}\}$ has to be verified
by applying \wikipedia{Mittag-Leffler's theorem}.
First take the difference $D(z,s) = F(z,s) - \tilde{F}(z,s)$, which is an entire function,
since the singularities are removed by substracting the principal part.
Next, we make use of \wikipedia{Liouville's theorem (complex analysis)},
by checking that $D(z,s)$ is bounded.
If it is bounded, then it means that $D(z,s)$ does not depend on $s$, that is $D(z,s) = f(z)$,
which means that $F(z,s) = f(z) + \tilde{F}(z,s)$.
If we are even more lucky, we may be able to find that $f(z) = 0$.

Below: How to find the principal parts of $\tilde{G}(z,s)$ and $\tilde{G}(z,s)^{-1}$.

\begin{proof}
	First recall the product expansions of $\sinh()$ and $\cosh()$
	\cite[{Eqs. (\dlmf[E]{4.36.}{1})} and {(\dlmf[E]{4.36.}{2})}]{dlmf}
	\begin{subequations}
		\begin{align}
		\sinh(\bm{u}) &=
		\bm{u} \prod_{k=1}^{+\infty} \left( 1 + \frac{\bm{u}^{2}}{k^{2} \pi^{2}} \right)
		\\
		\cosh(\bm{u}) &=
		\prod_{\ell=1}^{+\infty} \left(
		1 + \frac{4 \bm{u}^{2}}{(2\ell - 1)^{2} \pi^{2}}
		\right)
		\end{align}
	\end{subequations}
	and replace them in the expression for $G(z,s)$ and $G(z,s)^{-1}$ Eq. (\ref{coplanar:eqn:G}).	
	\begin{subequations}
		\begin{align}
			G(z,s) &=
			\frac{
				\cosh(\sqrt{s}\,z)/H
			}{
				\displaystyle
				s \prod_{k=1}^{+\infty} \left( 1 + \frac{s H^{2}}{k^{2} \pi^{2}} \right)
			}
			\\
			G(z,s)^{-1} &=
			\frac{
				\sqrt{s} \sinh(\sqrt{s}\, H)
			}{
				\displaystyle
				\prod_{\ell=1}^{+\infty} \left(
				1 + \frac{4s\, z^{2}}{(2\ell - 1)^{2} \pi^{2}}
				\right)
			}
		\end{align}
	\end{subequations}
	Here one can notice that both expressions have only real poles of multiplicity one
	\begin{subequations}
		\begin{align}
			s_{k} &= -k^{2} \frac{\pi^{2}}{H^{2}},& k &= 0, 1, 2, \ldots
			\\
			s_{\ell} &= -(2\ell - 1)^{2} \frac{\pi^{2}}{4z^{2}},& \ell &= 1, 2, \ldots
		\end{align}
	\end{subequations}
	where $s_{k}$ correspond to the poles of $G(z,s)$ and
	$s_{\ell}$ correspond to the poles of $G(z,s)^{-1}$
	(which are also the zeros of $G(z,s)$).
	This leads to the following partial fractions expansion
	\begin{subequations}
		\begin{align}
			\tilde{G}(z,s) &= \sum_{k=0}^{+\infty} \frac{A_{k}}{s - s_{k}}, &
			A_{k} &= \lim_{s \to s_{k}} (s - s_{k}) G(z,s)
			\\
			\tilde{G}(z,s)^{-1} &= \sum_{\ell=1}^{+\infty} \frac{B_{\ell}}{s - s_{\ell}}, &
			B_{\ell} &= \lim_{s \to s_{\ell}} (s - s_{\ell}) G(z,s)^{-1}
		\end{align}
	\end{subequations}
	Taking their inverse Laplace transform leads to
	\begin{subequations}
		\begin{align}
			g(z,t) = \laplace^{-1} \tilde{G}(z,s)
			&= \sum_{k=0}^{+\infty} A_{k} \e^{s_{k} t}
			\\
			h(z,t) = \laplace^{-1} \tilde{G}(z,s)^{-1}
			&= \sum_{\ell=1}^{+\infty} B_{\ell} \e^{s_{\ell} t}
		\end{align}
	\end{subequations}
	This completes the main proof.
	The rest of the proof consists of computing the coefficients $A_{k}$ and $B_{\ell}$.

	The coefficient $A_{0}$ can be calculated directly taking the limit
	\begin{subequations}
		\begin{align}
			A_{0} &= \lim_{s \to 0} s
			\frac{
				\cosh(\sqrt{s}\, z)
			}{
				\sqrt{s} \sinh(\sqrt{s}\, H)
			}
			= \lim_{s \to 0} \frac{1}{H}
			\frac{
				\cosh(\sqrt{s}\, z)
			}{
				\sinh(\sqrt{s}\, H)/(\sqrt{s}\, H)
			}
			\\
			A_{0} &= \frac{1}{H}
		\end{align}
	\end{subequations}
	and the remaining coefficients $A_{k}$ and $B_{\ell}$ can be computed by using L'Hôpital rule as follows
	\begin{subequations}
		\begin{align}
			A_{k} &= \lim_{s \to s_{k}} (s - s_{k})
			\frac{
				\cosh(\sqrt{s}\, z)
			}{
				\sqrt{s} \sinh(\sqrt{s}\, H)
			}
			\\
			&= \lim_{s \to s_{k}}
			\frac{
				\cosh(\sqrt{s}\, z) + (s - s_{k}) \deriv{}{s} \cosh(\sqrt{s}\, z)
			}{
				\num{0,5} H \sinh(\sqrt{s}\, H) / (\sqrt{s}\, H)
				+ \num{0,5} H \cosh(\sqrt{s}\, H)
			}
			\\
			&= \frac{2}{H}
			\frac{
				\cosh(\sqrt{s_{k}}\, z)
			}{
				\cosh(\sqrt{s_{k}}\, H)
			}
			= \frac{2}{H}
			\frac{
				\cos(\sqrt{|s_{k}|}\, z)
			}{
				\cos(\sqrt{|s_{k}|}\, H)
			}
			= \frac{2}{H}
			\frac{
				\cos(\sqrt{|s_{k}|}\, z)
			}{
				(-1)^{k}
			}
			\\
			&= \frac{2}{H} (-1)^{k} \cos(\sqrt{|s_{k}|}\, z)
		\end{align}
	\end{subequations}

	\begin{subequations}
		\begin{align}
			B_{\ell} &= \lim_{s \to s_{\ell}} (s - s_{\ell})
			\frac{
				\sqrt{s} \sinh(\sqrt{s}\, H)
			}{
				\cosh(\sqrt{s}\, z)
			}
			\\
			&= \lim_{s \to s_{\ell}}
			\frac{
				\sqrt{s} \sinh(\sqrt{s}\, H)
				+ (s - s_{\ell}) \deriv{}{s} \sqrt{s} \sinh(\sqrt{s}\, H)
			}{
				\num{0,5}z \sinh(\sqrt{s}\, z) / \sqrt{s}
			}
			\\
			&= \lim_{s \to s_{\ell}}
			\frac{
				2s \sinh(\sqrt{s}\, H)
			}{
				z \sinh(\sqrt{s}\, z)
			}
			= \frac{2}{z} s_{\ell} \frac{
				\sinh(\sqrt{s_{\ell}}\, H)
			}{
				\sinh(\sqrt{s_{\ell}}\, z)
			}
			\\
			&= \frac{2}{z} s_{\ell} \frac{
				\sin(\sqrt{|s_{\ell}|}\, H)
			}{
				\sin(\sqrt{|s_{\ell}|}\, z)
			}
			= \frac{2}{z} s_{\ell} \frac{
				\sin(\sqrt{|s_{\ell}|}\, H)
			}{
				(-1)^{\ell-1}
			}
			\\
			&= \frac{2}{z} |s_{\ell}| (-1)^{\ell} \sin(\sqrt{|s_{\ell}|}\, H)
		\end{align}
	\end{subequations}
\end{proof}
